A Modular Multimodal Architecture for Gaze Target Prediction: Application to Privacy-Sensitive Settings

Predicting where a person is looking is a complex task, requiring to understand not only the person's gaze and scene content, but also the 3D scene structure and the person's situation (are they manipulating? interacting or observing others? attentive?) to detect obstructions in the line of sight or apply attention priors that humans typically have when observing others. In this paper, we hypothesize that identifying and leveraging such priors can be better achieved through the exploitation of explicitly derived multimodal cues such as depth and pose. We thus propose a modular multimodal architecture allowing to combine these cues using an attention mechanism. The architecture can naturally be exploited in privacy-sensitive situations such as surveillance and health, where personally identifiable information cannot be released. We perform extensive experiments on the GazeFollow and VideoAttentionTarget public datasets, obtaining state-of-the-art performance and demonstrating very competitive results in the privacy setting case.

==> model-architecture-old.tex <==

We propose an image based model that predicts the attention location of a person given a single image or video frame. Our model consists of three parts - a Feature Extractor module for each modality, a Human-Centric module and an Attention module. We attach an additional In-Out module when we would like to predict whether a person is looking inside or outside the frame.

The modular nature of our architecture with separate feature extractors for each modality followed by late fusion allows us to add more modalities without having to retrain the whole model. At the same, the attention mechanism gives us insight into the importance of each modality while also allowing us to use a variable number of modalities. The combined model is illustrated in Figure~\ref{fig:full-model}.

\begin{figure*}
\centering
\includegraphics[width=0.9\textwidth]{latex/graphics/multimodal-gaze-architecture-smaller.png}
\caption{Overview of our proposed architecture.}
\label{fig:full-model}
\end{figure*}

\subsection{Human-Centric Module}

\subsection{Feature Extractor Modules}
\label{sec: feature-extractor}

The feature extractor is composed of an EfficientNet~\cite{tan2019efficientnet} backbone, pretrained on Imagenet~\cite{russakovsky2015imagenet} for classification. We use the Efficientnet models as they provide some of the best model size to accuracy trade-offs and come in different sizes ranging from the smallest (EfficientNet-b0) with 5.3M parameters to the largest (EfficientNet-b7) with 66M parameters. Given an input of shape $(H, W)$, it produces features of spatial resolution $(\frac{H}{4}, \frac{W}{4}), ... (\frac{H}{32}, \frac{W}{32})$. We combine these features using a Feature Pyramid Network~\cite{lin2017fpn} to produce a representative feature map of resolution $(\frac{H}{4}, \frac{W}{4})$. The Feature Pyramid Network uses skip connections from the high resolution representations during the upsampling process. This is in contrast to previous works that simply upsample the low resolution representations\cite{lian2018believe}\cite{chong2020dvisualtargetattention}. We show the importance of the skip connections in our ablation study~\ref{}.

Each feature extractor $\phi_i$ takes as input the modality $M_i$, the predicted gaze cone $G$ and a binary mask indicating the location of the person's head $H$ to give a feature map $F_i$.
\begin{equation}
    F_i = \phi_i (M_i \oplus G \oplus H)
\end{equation}
where $\oplus$ is the concatenation operator.

For training the feature extractor as well as for evaluating the informativeness of a single modality, we attach a prediction head $\rho_i$. It consists of upsampling and dilated convolution layers. The prediction head takes as input the feature maps $F_i$ to predict the gaze target heatmap $A^{pred}$. 
\begin{equation}
    A^{pred} = \rho_i (F_i)
\end{equation}

\subsection{Attention Module}
\label{sec: attention-module}

The goal of the attention module is to take the sequence of feature maps $F_i$ from each modality and produce a single combined feature map $F_v$ from which we can regress the attention map. This is in contrast to the standard transformer based self attention mechanism where the input and output both are sequences~\cite{vaswani2017attention}. We generate a single scalar weight $w_i$ for each modality and perform a weighted sum of the feature maps $F_i$ to produce $F_v$.
\begin{equation}
    F_v = \sum_{i=1}^n w_i F_i
\end{equation}

This attention mechanism allows us to use a variable number of modalities as the model can simply assign a weight of $0$ when a modality is absent. To encourage this behaviour, we perform modality dropout during training, i.e. we randomly provide a white noise image instead of the modality, and use an attention loss~[\ref{sec: loss}].

To generate the weights, each feature map $F_i$ is passed through a compression network $\kappa_i$ consisting of strided convolutions and max pooling to aggregate over the spatial dimension. This gives us an embedding vector $E_i$.
\begin{equation}
    E_i = \kappa_i(F_i)
\end{equation}
where $F_i$ $\in$ $\mathcal{R}^{\frac{H}{4} \times \frac{W}{4} \times D}$ and $E_i$ $\in$ $\mathcal{R}^D$.

The embedding vectors are concatenated and passed through a projection layer $P$ followed by softmax to get the attention weights $\{w_i\}_1^n$.
\begin{equation}
    \{w_i\}_1^n = \text{softmax}(P(E_1 \oplus E_2 . . . \oplus E_n))
\end{equation}

The gaze target heatmap $A^{pred}$ is regressed from the combined feature map $F_v$ using a prediction head~[\ref{sec: feature-extractor}] $\rho_A$.
\begin{equation}
    A^{pred} = \rho_A(F_v)
\end{equation}

\subsection{In-Out Module}

We attach an In-Out module when we would like to predict whether a person is looking inside or outside the frame. This is important as we do not want to use the gaze target prediction when a person is looking outside the frame. The In-Out module consists of linear layers followed by a sigmoid activation. It takes the combined feature map $F_v$ from the attention module and the head embedding $HE$ from the human-centic module to classify whether a person is looking inside or outside the frame.
\begin{equation}
    IO = \theta (F_v \oplus HE)
\end{equation}

\subsection{Loss}
\label{sec: loss}

The complete model~\ref{} is trained end-to-end using a combination of four losses.

$\mathcal{L}_{gaze}$ computes the pixel-wise L2 loss between the predicted gaze target heatmap $A^{pred}$ and the ground truth gaze target heatmap $A^{gt}$. $\mathcal{L}_{dir}$ maximizes the cosine of the angle between the predicted direction vector $(g_x^{pred}, g_y^{pred})$ and the ground truth direction vector $(g_x^{gt}, g_y^{gt})$. $\mathcal{L}_{in-out}$ is the binary cross entropy loss for whether a person is looking inside or outside the frame. 
% \begin{equation}
%     \mathcal{L}_{gaze} = \frac{16}{H \times W} \sum_{x}\sum_{y} (A^{pred}_{x,y} - A^{gt}_{x,y})^2
% \end{equation}
% \begin{equation}
%     \mathcal{L}_{dir} = 1 - \frac{(g_x^{pred}, g_y^{pred}).(g_x^{gt}, g_y^{gt})}{||(g_x^{pred}, g_y^{pred})||_2.||(g_x^{gt}, g_y^{gt})||_2}
% \end{equation}

Additionally, we use an attention loss $\mathcal{L}_{att}$. The attention loss provides weak supervision to the attention module. As described in Section ~\ref{sec: attention-module}, we would like the attention score for a modality to be $0$ when it is not present. By performing modality dropout, we know the modality dropped during training. $\mathcal{L}_{att}$ pushes the attention score for the dropped modalities to $0$.
\begin{equation}
    \mathcal{L}_{att} = \sum_{i=1}^{n} w_i . \mathbbm{1}_{i \in \text{dropped}}
\end{equation}
where $\mathbbm{1}$ is an indicator variable and 'dropped' is the list of modalities dropped.

The final loss is a linear combination of the four losses:
\begin{equation}
    \mathcal{L} = \lambda_{gaze} \mathcal{L}_{gaze} + \lambda_{dir} \mathcal{L}_{dir} + \lambda_{in-out} \mathcal{L}_{in-out} + \lambda_{att} \mathcal{L}_{att}
\end{equation}

==> sec_acknowledgement.tex <==
\section{Acknowledgment}

This research has been supported by the ROSALIS project (Robot skills acquisition through active learning and social interaction strategies, grant agreement no. 30214) of the Swiss National Science Foundation (SNSF) as well as by the AI4Autism project (Digital Phenotyping of Autism Spectrum Disorders in children, grant agreement no. CRSII5\_202235 / 1) of the the Sinergia interdisciplinary program of the SNSF. 
